Robust Graph Embedding with Noisy Link Weights

We propose $\beta$-graph embedding for robustly learning feature vectors from data vectors and noisy link weights. A newly introduced empirical moment $\beta$-score reduces the influence of contamination and robustly measures the difference between the underlying correct expected weights of links and the specified generative model. The proposed method is computationally tractable; we employ a minibatch-based efficient stochastic algorithm and prove that this algorithm locally minimizes the empirical moment $\beta$-score. We conduct numerical experiments on synthetic and real-world datasets.

==> preamble.tex <==
\renewcommand{\kanjifamilydefault}{\gtdefault} % 日本語書体をゴシック体に
\renewcommand{\familydefault}{\sfdefault} % 欧文書体をHelveticaに




%%% packages
\usepackage{latexsym}
\usepackage{amsmath,amssymb}
\usepackage{bm}
\usepackage[dvipdfmx]{graphicx}
\usepackage{float}
\usepackage{ascmac}
\usepackage{color}
\usepackage{enumerate}
\usepackage{comment}
\usepackage{wrapfig}
\usepackage{here}
\usepackage{mathrsfs}
\usepackage[top=20truemm,bottom=20truemm,
	left=25truemm,right=25truemm]{geometry}


%% しおりを作る
\usepackage[dvipdfmx]{hyperref}
\usepackage{pxjahyper} %%hyperref読み込みの直後に




\setcounter{tocdepth}{3}
\renewcommand{\appendixname}{}
\def\mybf#1{\mbox{\boldmath $#1$}}


  \makeatletter
  \renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
  \@addtoreset{equation}{section}
  \makeatother



%%% symbol of Q.E.D.
\def\qed{\hfill $\Box$} 

%%% standard mathematical symbols
\newcommand{\diff}{\mathrm{d}} 
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\fixed}{\mathrm{:fixed}}
\newcommand{\otherwise}{\mathrm{otherwise}}
\newcommand{\zero}{\boldsymbol 0}
\newcommand{\rank}{\mathrm{rank}}

%%% symbols for matrix
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\mode}{\mathbf{mode}}

%%% symbols for r.v.s
\newcommand{\ave}{\text{E}}
\newcommand{\prob}[1]{\text{P}\left[#1\right]}
\newcommand{\var}[1]{\text{V}\left[#1\right]}
\newcommand{\cov}[1]{\text{Cov}\left[#1\right]}
\newcommand{\cor}[1]{\text{Cor}\left[#1\right]}

%%% symbols for boldsymbols
\newcommand{\bs}{\boldsymbol} 
\newcommand{\x}{\bs x}
\newcommand{\X}{\bs X}
\newcommand{\y}{\bs y}
\newcommand{\Y}{\bs Y}
\newcommand{\iid}{\mathrm{i.i.d.}}



%%% symbols for argmin series
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argsolve}{arg\,solve}
\newcommand{\argmin}{\mathop{\rm arg.~min.}}
\newcommand{\argmax}{\mathop{\rm arg.~max.}}
\newcommand{\argsolve}{\mathop{\rm arg.~min.}}


\newtheorem{ex}{Ex.}[section]

\newtheorem{theo}{Theorem}[section]
\newtheorem{lem}[theo]{Lemma}
\newtheorem{prop}[theo]{Proposition}
\newtheorem{defi}[theo]{Definition}
\newtheorem{proof}{Proof}[section]
\newtheorem{cond}{Condition}[section]

\newtheorem{remark}{Remark}[section]


\renewcommand{\abstractname}{{\Large 概要|}}



